T\^atonnement in Homothetic Fisher Markets

A prevalent theme in the economics and computation literature is to identify natural price-adjustment processes by which sellers and buyers in a market can discover equilibrium prices. An example of such a process is t\^atonnement, an auction-like algorithm first proposed in 1874 by French economist Walras in which sellers adjust prices based on the Marshallian demands of buyers. A dual concept in consumer theory is a buyer's Hicksian demand. In this paper, we identify the maximum of the absolute value of the elasticity of the Hicksian demand, as an economic parameter sufficient to capture and explain a range of convergent and non-convergent t\^atonnement behaviors in a broad class of markets. In particular, we prove the convergence of t\^atonnement at a rate of $O((1+\varepsilon^2)/T)$, in homothetic Fisher markets with bounded price elasticity of Hicksian demand, i.e., Fisher markets in which consumers have preferences represented by homogeneous utility functions and the price elasticity of their Hicksian demand is bounded, where $\varepsilon \geq 0$ is the maximum absolute value of the price elasticity of Hicksian demand across all buyers. Our result not only generalizes known convergence results for CES Fisher markets, but extends them to mixed nested CES markets and Fisher markets with continuous, possibly non-concave, homogeneous utility functions. Our convergence rate covers the full spectrum of nested CES utilities, including Leontief and linear utilities, unifying previously existing disparate convergence and non-convergence results. In particular, for $\varepsilon = 0$, i.e., Leontief markets, we recover the best-known convergence rate of $O(1/T)$, and as $\varepsilon \to \infty$, e.g., linear Fisher markets, we obtain non-convergent behavior, as expected.

==> equivalence.tex <==
\section{Equivalence of Generalized Gradient Descent and T\^atonnement}
\label{sec:equiv}

\citeauthor{fisher-tatonnement} \cite{fisher-tatonnement} have shown via the Lagrangian of the Eisenberg-Gale program, i.e., without constructing the dual exactly, that the subdifferential of the dual of the Eisenberg-Gale program %\amy{it's a bit weird that they were able to show this, since the dual was not known. maybe add a footnote that their dual also differed from the actual EG dual by a constant factor?}\deni{But they did not know the dual! they just used a proof by cases using the Lagrangian.}
is equal to the negative excess demand in the associated market, which implies that (generalized) gradient descent equivalent to a subset of t\^atonnement rules.
In this section, we use a generalization of Shephard's lemma to prove that the subdifferential of the dual of our new convex program is equal to the negative excess demand in the associated market.
Our proof also applies to the dual of the Eisenberg-Gale program, since the two duals differ only by a constant factor.

Shephard's lemma tells us that the rate of change in expenditure with respect to prices, evaluated at prices $\price$ and utility level $\goalutil[\buyer]$, is equal to the Hicksian demand at prices $\price$ and utility level $\goalutil[\buyer]$.
%\deni{This is wrong, previous lemma is a derivative with respect to the utility level, this is a derivative with respect to prices.} \deni{That said, what you are saying is correct for \textbf{strictly concave utility functions} but bit because of Shepherd's lemma; it is just a consequence of homogeneity.}
%
%\amy{the above comments are wrt total expenditure across all goods. the next sentence moves from subdifferentials to partials.}
%
%The proof of this lemma (in the case of strictly concave utility functions) uses the envelope theorem to show that
Alternatively, the partial derivative of the expenditure function with respect to the price $\price[\good]$ of good $\good$ at utility level $\goalutil[\buyer]$ is simply the share of the total expenditure allocated to $\good$ divided by the price of $\good$, which is exactly the Hicksian demand for $\good$ at utility level $\goalutil[\buyer]$.

While Shephard's lemma is applicable to utility functions with singleton-valued Hicksian demand (i.e., strictly concave utility functions), we require a generalization of Shephard's lemma that applies to utility functions that are not strictly concave and that could have set-valued Hicksian demand.
%To the best of our knowledge, 
An early proof of this generalized lemma was given by \citeauthor{generalized-shephard} in a discussion paper \cite{generalized-shephard};
a more modern perspective can be found in a recent survey by \citeauthor{duality-economics} \cite{duality-economics}.
For completeness, we also provide a new, simple proof of this result via Danskin's theorem (for subdifferentials) \cite{danskin1966thm}.

\begin{theorem}[Shephard's lemma, generalized for set-valued Hicksian demand \cite{duality-economics, shephard, generalized-shephard}]
\label{shepherd}
Let $\expend[\buyer](\price, \goalutil[\buyer])$ be the expenditure function of buyer $\buyer$ and $\hicksian[\buyer](\price, \goalutil[\buyer])$ be the Hicksian demand set of buyer $\buyer$.
The subdifferential $\subdiff[{\price}] \expend[\buyer](\price, \goalutil[\buyer])$ is the Hicksian demand at prices $\price$ and utility level $\goalutil[\buyer]$, i.e., $\subdiff[\price] \expend[\buyer](\price, \goalutil[\buyer]) = \hicksian[\buyer](\price, \goalutil[\buyer])$.
%That is, $\bm{\chi}_\buyer \in \subdiff[{\price}] \expend[\buyer](\price, \goalutil[\buyer])$ iff $\bm{\chi}_{\buyer} \in \hicksian[\buyer](\price, \goalutil[\buyer])$.
%\amy{i like this notation, without the fraction, better. why don't we use it everywhere -- instead of fractions.}\deni{I avoid using it in cases where the object is supposed to not be a set, I guess we could abuse notation but we should say it somehwere if you prefer that.}
\end{theorem}


\begin{proof}
%[\cref{shepherd}]
Recall that $\expend[\buyer](\price, \goalutil[\buyer]) = \min_{\x \in \R^\numgoods_+ : \util[\buyer](\x) \geq \goalutil[\buyer]} \price \cdot \x$.
Without loss of generality, we can assume that consumption set is bounded from above, since utilities are assumed to represent locally non-satiated preferences, i.e., $ \min_{\x \in X : \util[\buyer](\x) \geq \goalutil[\buyer]} \price \cdot \x$ where $X \subset \R^\numgoods_+$ is compact.
Using Danskin's theorem:
%
\begin{align*}
    \subdiff[\price] \expend[\buyer](\price, \goalutil[\buyer]) &= \left\{  \grad[\price] \left( \price \cdot \x \right)(\x^*(\price, \goalutil[\buyer])) \mid \x^*(\price, \goalutil[\buyer]) \in \hicksian[\buyer](\price, \goalutil[\buyer])\right\} && \text{(Danskin's Theorem)} \\
    &= \left\{  \x^*(\price, \goalutil[\buyer]) \mid \x^*(\price, \goalutil[\buyer]) \in \hicksian[\buyer](\price, \goalutil[\buyer])\right\} \\
    &= \hicksian[\buyer](\price, \goalutil[\buyer])
\end{align*}

\noindent
The first equality follows from Danskin's theorem, using the facts that the objective of the expenditure minimization problem is affine and the constraint set is compact.
The second equality follows by calculus, and the third, by the definition of Hicksian demand.
\end{proof}

The next lemma plays an essential role in the proof that the subdifferential of the dual of our convex program is equal to the negative excess demand.
% \amy{see the two remarks below this lemma. it seems to play an essential role in much more than just what we say in this sentence! can we expand on its importance?}\deni{I like the below two lemmas but I am not sure adding more here will be providing much value?}
Just as Shephard's Lemma related the expenditure function to Hicksian demand via (sub)gradients, this lemma relates the expenditure function to Marshallian demand via (sub)gradients.
%
One way to understand this relationship is in terms of \mydef{Marshallian consumer surplus},
%\amy{except that the reader has no intuition for consumer surplus :(} 
the area under the Marshallian demand curve, i.e., the integral of Marshallian demand with respect to prices.%
\footnote{We note that the definition of Marshallian consumer surplus for multiple goods requires great care and falls outside the scope of this paper. More information on consumer surplus can be found in \citeauthor{levin-notes} \cite{levin-notes}, and \citeauthor{vives1987marshallian} \cite{vives1987marshallian}.}
Specifically, by applying the fundamental theorem of calculus to the left-hand side of \Cref{lemma-deriv-marshallian}, we see that the Marshallian consumer surplus equals $\budget[\buyer] \log \left(\partderiv[{\expend[\buyer](\price, \goalutil[\buyer])}][{\goalutil[\buyer]}] \right)$.
%
The key takeaway of this lemma is thus that any objective function we might seek to optimize that includes a buyer's Marshallian consumer surplus is thus optimizing their Marshallian demand, so that optimizing this objective yields a utility-maximizing allocation for the buyer, constrained by their budget.

\begin{lemma}
\label{lemma-deriv-marshallian}
If buyer $\buyer$'s utility function $\util[\buyer]$ is CCH,
%Let $\expend[\buyer](\price, \goalutil[\buyer])$ be the expenditure function of buyer $\buyer$ and let $\marshallian[\buyer](\price, \budget[\buyer])$ be the Marshallian demand of buyer $\buyer$.
then
%\begin{align}
$\subdiff[\price] \left( 
    \budget[\buyer] \log \left(\partderiv[{\expend[\buyer](\price, \goalutil[\buyer])}][{\goalutil[\buyer]}]  \right) \right) = 
    \marshallian[\buyer](\price, \budget[\buyer])$.
%   \enspace .
%\end{align}
\end{lemma}

\begin{proof}
%[Proof of \Cref{lemma-deriv-marshallian}]
Without loss of generality, we can assume $\util[\buyer]$ is homogeneous of degree 1. Then:
\begin{align*}
    \subdiff[\price] \left( 
    \budget[\buyer] \log \left(\partderiv[{\expend[\buyer](\price, \goalutil[\buyer])}][{\goalutil[\buyer]}] \right) \right)
    &= \left( \frac{\budget[\buyer]}{\partderiv[{\expend[\buyer](\price, \goalutil[\buyer])}][{\goalutil[\buyer]}]} \right) \subdiff[\price] \left( 
    \partderiv[{\expend[\buyer](\price, \goalutil[\buyer])}][{\goalutil[\buyer]}] \right) && \text{(Derivative of the logarithm)} \\
    &= \budget[\buyer] \left( \partderiv[{\indirectutil[\buyer](\price, \budget[\buyer])}][{\budget[\buyer]}] \right) \subdiff[\price] \left( \partderiv[{\expend[\buyer](\price, \goalutil[\buyer])}][{\goalutil[\buyer]}] \right) && \text{(\Cref{inverse-expend})} \\
    &= \budget[\buyer] \left( \partderiv[{\indirectutil[\buyer](\price, \budget[\buyer])}][{\budget[\buyer]}] \right) \subdiff[\price]
    \expend[\buyer](\price, 1) && \text{(\Cref{derive-expend})} \\
    &= \budget[\buyer] \left( \partderiv[{\indirectutil[\buyer](\price, \budget[\buyer])}][{\budget[\buyer]}] \right) \hicksian[\buyer](\price, 1) && \text{(Shephard's Lemma)} \\
    &= \budget[\buyer] \, \indirectutil[\buyer](\price, 1) \, \hicksian[\buyer](\price, 1) && \text{(\Cref{deriv-indirect-util})} \\
    &=  \indirectutil[\buyer](\price, \budget[\buyer]) \, \hicksian[\buyer](\price, 1) && \text{(\Cref{homo-indirect-util})} \\
    &=  \hicksian[\buyer]\left(\price, \indirectutil[\buyer](\price, \budget[\buyer]) \right) && \text{(\Cref{homo-expend})} \\
    &=  \marshallian[\buyer](\price, \budget[\buyer]) && \text{(\Cref{hicksian-marshallian})}
\end{align*}
\end{proof}
% \amy{seems like Lemma 4 should move as well, since it is not needed above!}

\begin{remark}
\Cref{lemma-deriv-marshallian} makes the dual of our convex program easy to interpret,
%the objective function of 
and thus sheds light on the dual of the Eisenberg-Gale program.
%%%
%, which had previously eluded us.
\if 0
Consider the sub-expression $- \sum_{\buyer \in \buyers} \budget[\buyer] \log{ \left(\partderiv[{\expend[\buyer](\price, \goalutil[\buyer])}][{\goalutil[\buyer]}] \right)}$.
Since the utility functions are assumed to be CCH, maximizing the budget-weighted logarithm of the marginal cost of utility is equivalent to maximizing the Marshallian demand, or the total of the buyers' utilities constrained by their budgets (\Cref{lemma-deriv-marshallian}).
Second, consider the sub-expression $\sum_{\good \in \goods} \price[\good]$.
Minimizing prices is equivalent to calibrating prices such that the market clears.
Hence, the objective function can be seen as the efforts of a fictional auctioneer who is trying to maximize the utility of each buyer constrained by their budget, while controlling prices so that the market clears. \amy{i am missing the market clearing intuition. i like the next intuition better, about minimizing distance. maybe i need to see some examples. is there a way to interpret the VALUE of our convex program?}
\fi
%
Specifically, we can interpret the dual as minimizing the distance between the sellers' and the buyers' surplus.
The left hand term is simply the sellers' surplus, and by \Cref{lemma-deriv-marshallian}, the right hand term can be seen as the buyers' total Marshallian surplus.
\end{remark}

%\amy{when you find the dual, you abstract out the computation of the primal---the allocation. and likewise, for the primal. so there is a separation of concerns. need to argue why the two claims above about optimizing buck per bang or bang per buck lead to separation of concerns.}

\begin{remark}
The lemmas we have proven in this section and the last provide a possible explanation as to why no primal-dual type
%\amy{remind me why we added the ``primal-dual'' qualifier. do we need it?}\deni{Yes, we need it. because a convex program to solve for prices on their own might exists, but this might not mean that its dual will gives equilibrium allocations necessarily}
convex program is known that solves Fisher markets when buyers have \emph{non-homogeneous\/} utility functions, in which the primal describes optimal allocations while the dual describes equilibrium prices.
%
By the homogeneity assumption, a CCH buyer can increase their utility level (resp. decrease their spending) by $c\%$ by increasing their budget (resp. decreasing their desired utility level) by $c\%$ (\Cref{homo-indirect-util}).
This observation implies that the marginal expense of additional utility, i.e., ``bang-per-buck'', and the marginal utility of additional budget, i.e., ``buck-per-bang'', are constant (\Cref{deriv-indirect-util}).
Additionally,  optimizing prices to maximize buyers'  ``bang-per-buck'' is equivalent to optimizing prices to minimize their ``buck-per-bang'' (\Cref{inverse-expend}).
Further, optimizing prices to minimize their ``buck-per-bang'' is equivalent to maximizing their utilities constrained by their budgets (\Cref{lemma-deriv-marshallian}).
Thus, the equilibrium prices computed by the dual of our program, which optimize the buyers' buck-per-bang, simultaneously optimize their utilities constrained by their budgets.
%
In particular, equilibrium prices can be computed without reference to equilibrium allocations (\Cref{inverse-expend} + \Cref{lemma-deriv-marshallian}).
In other words, assuming homogeneity, the computation of the equilibrium allocations and prices can be isolated into separate primal and dual problems.
\end{remark}

We now show that the subdifferential of the dual of our convex program is equal to the negative excess demand in the associated market.

\begin{theorem}
\label{excess-demand}
The subdifferential of the dual of the program given in \Cref{new-convex} for a CCH Fisher market $(\util, \budget)$ at any price $\price$ is equal to the negative excess demand in $(\util, \budget)$ at price $\price$:
%
\begin{align}   
    \subdiff[\price] \left( \sum_{\good \in \goods} \price[\good] - \sum_{\buyer \in \buyers} \budget[\buyer] \log{ \partial_{\goalutil[\buyer]}{\expend[\buyer] (\price, \goalutil[\buyer])}} \right) 
    % = \bm{1}_{\numgoods} - \sum_{\buyer \in \buyers} \marshallian[\buyer](\price, \budget[\buyer]) 
    = - \excess(\price)
\end{align}
\end{theorem}

\begin{proof}
% \sdeni{Since the utility functions are continuous, concave, and represent locally non-satiated preferences, $\expend[\buyer](\price, \goalutil[\buyer])$ is continuous and concave in $\price$ \cite{levin-notes, mas-colell}. Moreover, the derivative of the expenditure function with respect to the utility level, namely $\expend[\buyer](\price, 1)$, is also continuous and concave.
% Since the logarithm is also a concave function, and the composition of two concave functions remains concave,
% $-\sum_{\buyer \in \buyers} \budget[\buyer] \log{ \left(\partderiv[{\expend[\buyer](\price, \goalutil[\buyer])}][{\goalutil[\buyer]}] \right)}$ is convex, ensuring that the objective function is also convex, since $\sum_{\good \in \goods} \price[\good]$ is affine.
% Hence, the minimum of this objective function is well-defined.

% The first-order optimality condition of our convex program is that the subdifferential of the objective function contains 0 at an optimal solution $\price^*$.
% But then,}{} 
For all goods $\good \in \goods$, we have:
\begin{align*}
    &\subdiff[{\price[\good]}] \left(\sum_{\good \in \goods} \price[\good] - \sum_{\buyer \in \buyers} \budget[\buyer] \log{ \partial_{\goalutil[\buyer]}{\expend[\buyer] (\price, \goalutil[\buyer])}} \right) \\
    &=\{1\} - \subdiff[{\price[\good]}] \left(\sum_{\buyer \in \buyers} \budget[\buyer] \log{ \partial_{\goalutil[\buyer]}{\expend[\buyer] (\price, \goalutil[\buyer])}} \right) \\
    &= \{1\} - \sum_{\buyer \in \buyers} \subdiff[{\price[\good]}] \left( \budget[\buyer] \log{ \partial_{\goalutil[\buyer]}{\expend[\buyer] (\price, \goalutil[\buyer])}} \right) \\
    &=\{1\} - \sum_{\buyer \in \buyers} \marshallian[\buyer][\good](\price, \budget[\buyer]) && \text{(\Cref{lemma-deriv-marshallian})} \\
    &= -\excess[\good](\price)
\end{align*}

% \noindent
% In other words, all of good $\good$ is demanded by the buyers in aggregate, so the market clears.
% Moreover, by the definition of the Marshallian demand, each buyer maximizes their utility constrained by their budget.
% Therefore, the solution $\price^*$ of our convex program is an equilibrium price vector of the Fisher market $(\util, \budget)$.
\end{proof}

%This theorem implies that the dual of our convex program is a convex potential function for CCH Fisher markets, a fact previously proven by \citeauthor{fisher-tatonnement} for the dual of the Eisenberg-Gale program for which no explicit dual formulation was known.

\citeauthor{fisher-tatonnement} \cite{fisher-tatonnement} define a class of markets called \mydef{convex potential function (CPF)} markets.
A market is a CPF market, if there exists a convex potential function $\varphi$ such that $\subdiff[\price] \varphi(\price) = - \excess(\price)$.
They then prove that Fisher markets are CPF markets by showing, through the Lagrangian of the Eisenberg-Gale program, that its dual is a convex potential function \cite{fisher-tatonnement}.
Likewise, \Cref{excess-demand} implies the following:

\begin{corollary}
All CCH Fisher markets are CPF markets.
\end{corollary}

\begin{proof}
A convex potential function $\phi: \mathbb{R}^{\numgoods} \to \mathbb{R}$ for any CCH Fisher market $(\util, \budget)$ is given by:
%
\begin{align}
    \potential (\price) = \sum_{\good \in \goods} \price[\good] - \sum_{\buyer \in \buyers} \budget[\buyer] \log{ \left( \partderiv[{\expend[\buyer] (\price, \goalutil[\buyer])}][{\goalutil[\buyer]}] \right)}\label{potential-func}
\end{align}
\end{proof}

Fix a kernel function $h$ for the Bregman divergence $\divergence[h]$.
If the generalized gradient descent procedure given in  \Crefrange{generalized-descent}{generalized-descent2} is run on \Cref{potential-func} (i.e., choose $f = \potential$), it is equivalent to the t\^atonnement process for some monotonic function of the excess demand \cite{fisher-tatonnement}:
%
\begin{align}
    \price(t+1) = \min_{\price \in \mathbb{R}^\numgoods} \left\{ \price(t) +  \subgrad(t)\left(\price - \price(t) \right) + \gamma_t \divergence[\mathrm{h}][\price][\price(t)] \right\}  && \text{for } t = 0, 1, 2, \hdots\\
    \subgrad(t) \in \subdiff[\price] \potential(\price(t))\\
    \price(0) \in \mathbb{R}^\numgoods_+
\end{align}

\noindent
Thus, by varying the kernel function $h$ of the Bregman divergence we can obtain different t\^atonnement rules.
For instance, if $h = \frac{1}{2}||x||^2_2$, the generalized gradient descent process reduces to the classic t\^atonnement rule given by $G(\x) = \gamma_t \x$, for $\gamma_t > 0$ and for all $t \in \N$, in \Crefrange{tatonnement}{tatonnement2}.
Using this equivalence between generalized gradient descent and t\^atonnement, we can pick a particular kernel function $h$, and then potentially use \Cref{theorem-devanur} to establish convergence rates for t\^atonnement.


==> experiments.tex <==
\section{Experiments}

\citeauthor{fisher-tatonnement} \cite{fisher-tatonnement} proved a worst-case \emph{lower\/} bound of $\Omega(\nicefrac{1}{t^2})$ to complement their $O(\nicefrac{1}{t})$ worst-case upper bound for the convergence rate of entropic t\^atonnement in Leontief markets.
These results suggest a possible convergence rate of $\Omega(\nicefrac{1}{t^2})$.
%Our goals with our experiments are two-fold, to verify empirically that a sublinear convergence rate holds in CSCH Fisher markets, and 
The goal of these experiments is to see if it might be possible to improve upon the known worst-case convergence rate of $O(\nicefrac{1}{t})$ for entropic t\^atonnement in not only Leontief, but all CSCH Fisher markets.%
\footnote{Our code can be found on \coderepo.}

First, as a sanity check, we confirmed experimentally our analytically derived convergence rate.
To do so, we randomly initialized 10,000 mixed (strictly concave) CES Fisher markets with 10 buyers and 5 goods.
We assigned each buyer, uniformly at random, either CES, Cobb-Douglas, or Leontief utilities.
The buyers' values for goods, and their budgets, were drawn uniformly between 2 and 3.
For CES buyers, we chose the $\rho$ parameter uniformly at random in the range $[\nicefrac{1}{4}, \nicefrac{3}{4}] \cap [-1, -101]$.%
\footnote{We ruled out very small values of $\rho$, as well as values close to 0 or 1, to ensure numerical stability.}
We also drew initial prices uniformly in the range $[2,3]$.
We then ran the entropic t\^atonnement update rule in each market, and asked whether the process ever converged at a rate worse than sublinear. \emph{We found no such examples.}

On the contrary, the results depicted in \Cref{fig:obj_change} suggest that the sublinear convergence rate of $O(\nicefrac{1}{t})$ could be improved to $O(\nicefrac{1}{t^2})$ for entropic t\^atonnement.
%
(The inner frame in \Cref{fig:obj_change} is a closeup of iterations 0 to 10, intended to clarify that the average trajectory of the objective value throughout entropic t\^atonnement decreases at a rate faster than $O(\nicefrac{1}{t^2})$.)
%
Together with the known worst-case convergence lower bound of $\Omega(\nicefrac{1}{t^2})$ for Leontief Fisher markets \cite{fisher-tatonnement}, these experiments suggest that entropic t\^atonnement might have a tight convergence bound of $\Theta(\nicefrac{1}{t^2})$ in CSCH Fisher markets.

Additionally, to understand the behavior of t\^atonnement in mixed CCH (i.e., not necessarily strictly concave) Fisher markets, we ran almost the same experiment again, but this time, each buyer was assigned, uniformly at random, either CES, Cobb-Douglas, Leontief, or \emph{linear\/} utilities.
We then checked, for each market, if the process converged.
We found that out of 10,000 experiments, 9889 of them did \emph{not\/} converge.
We show a sample entropic t\^atonnement trajectory for one mixed CCH Fisher market in \Cref{fig:obj_change_linear}.
We see that the objective value decreases initially (at a rate slower than $\nicefrac{1}{t^2}$), but then, after about 10 iterations, it goes back up, and it continues to oscillate.
In other words, it seems the market tends toward an equilibrium, but is unable to settle at one.
This result is unsurprising since, in expectation, buyers with linear (i.e., non-CSCH) utilities make up a quarter of the market.

\begin{figure}[ht]
\centering
\begin{subfigure}[b]{0.475\textwidth}
    \centering
    \includegraphics[width=\textwidth]{graphs/obj_change.png}
    \caption{Average trajectory of the value of the objective function throughout t\^atonnement with KL divergence for CSCH Fisher markets is drawn in {\color{red} red}. The predicted worst case sublinear convergence rate is depicted by a dashed {\color{blue} blue} line. A convergence rate of $\nicefrac{1}{t^2}$ and $\nicefrac{1}{t^3}$ are denoted in {\color{green} green} and {\color{orange} orange}, respectively.}
    \label{fig:obj_change}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.475\textwidth}
    \centering
    \includegraphics[width=\textwidth]{graphs/obj_change_with_linear.png}
    \caption{Example trajectory of the value of the objective function throughout t\^atonnement with KL divergence for CCH Fisher markets is drawn in {\color{red} red}. The predicted worst case sublinear convergence rate is depicted by a dashed {\color{blue} blue} line. A convergence rate of $\nicefrac{1}{t^2}$ and $\nicefrac{1}{t^3}$ are denoted in {\color{green} green} and {\color{orange} orange}, respectively.}
    \label{fig:obj_change_linear}
\end{subfigure}
\end{figure}

==> figure1.tex <==

% \begin{figure}[ht!]
%     \centering
%     \begin{tikzpicture}[framed, scale=0.3, transform shape]
%           \node [venn circle = cyan, minimum size=2cm, scale= 2] (CES) at (5,-2) {\begin{tabular}{c}
%                {CES ($\rho < 1$)} \\
%                {$(1-\Theta(1))^t$}
%           \end{tabular} };
          
%           \node [venn circle = cyan, minimum size=2cm, scale=1.7] (leontief) at (7,2) {\begin{tabular}{c}
%                {Leontief} \\
%                {$O(\nicefrac{1}{t})$}
%           \end{tabular}};

%           \node [venn circle = magenta] (Homothetic) at (5,0) {};
%           \node [label, scale = 2] (CCHlabel) at (4,3.5) {\begin{tabular}{c}
%                {Homothetic} \\
%                {$O(\nicefrac{1 + \elastic^2}{t})$}
%           \end{tabular}};  
% %             
%           \node [venn circle = blue, minimum size=6.5cm] (WGS) at (0.5,0.5) {};
%           \node [label, scale = 1.5] (WGSlabel) at (-1.35, 0.75) {\begin{tabular}{c}
%                {WGS} \\
%                {$\left(1-\Theta(1)\right)^t$}
%           \end{tabular}};
          
%           \node [venn circle = blue, minimum size=6.5cm] (WGC) at (7.5, 0.75) {};
%           \node [label, scale = 1.5] (WGClabel) at (7.5, 0.75) {\begin{tabular}{c}
%                {WGC} \\
%                {$\left(1-\Theta(1)\right)^t$}
%           \end{tabular}};

%           \node [label] (title) at (-2,5){\Huge Space of Fisher markets};
%         %   \node [label, rotate=65] (WGSCES) at (3.25, -1.25) {CES with $\rho > 0$};
%           \node [label, scale = 2] (WGSCES) at (-1, -5) {CES with $\rho > 0$};
%           \draw[->] (WGSCES) -- (3.25, -1.25);
% \end{tikzpicture}
%     \caption{
%     % \scriptsize 
%     The convergence rates of t\^atonnement for different Fisher markets. We color previous contributions in blue, and our contribution in red, i.e., we study homothetic Fisher markets. We note that the convergence rate for WGS markets does not apply to markets where the price elasticity of Marshallian demand is unbounded, e.g., linear Fisher markets; likewise, the convergence rate for CES Fisher markets does not apply to linear Fisher markets.}
%     \label{fig:utility-functions}
% \end{figure}




 



% \begin{subfigure}
%     \centering
% \resizebox{0.5\columnwidth}{!}
% {

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp9047127948672036] 
\draw   (148,27) -- (559,27) -- (559,282) -- (148,282) -- cycle ;
%Shape: Circle [id:dp621497278386274] 
\draw  [color={rgb, 255:red, 184; green, 133; blue, 186 }  ,draw opacity=1 ][fill={rgb, 255:red, 184; green, 133; blue, 186 }  ,fill opacity=0.36 ][line width=3]  (240,154.5) .. controls (240,91.82) and (290.82,41) .. (353.5,41) .. controls (416.18,41) and (467,91.82) .. (467,154.5) .. controls (467,217.18) and (416.18,268) .. (353.5,268) .. controls (290.82,268) and (240,217.18) .. (240,154.5) -- cycle ;
%Shape: Circle [id:dp1249309213526526] 
\draw  [color={rgb, 255:red, 92; green, 152; blue, 210 }  ,draw opacity=1 ][fill={rgb, 255:red, 92; green, 152; blue, 210 }  ,fill opacity=0.35 ][line width=2.25]  (299.5,204.25) .. controls (299.5,172.91) and (324.91,147.5) .. (356.25,147.5) .. controls (387.59,147.5) and (413,172.91) .. (413,204.25) .. controls (413,235.59) and (387.59,261) .. (356.25,261) .. controls (324.91,261) and (299.5,235.59) .. (299.5,204.25) -- cycle ;
%Shape: Circle [id:dp3234953905347524] 
\draw  [color={rgb, 255:red, 92; green, 152; blue, 210 }  ,draw opacity=1 ][fill={rgb, 255:red, 92; green, 152; blue, 210 }  ,fill opacity=0.36 ][line width=2.25]  (390,140) .. controls (390,121.22) and (405.22,106) .. (424,106) .. controls (442.78,106) and (458,121.22) .. (458,140) .. controls (458,158.78) and (442.78,174) .. (424,174) .. controls (405.22,174) and (390,158.78) .. (390,140) -- cycle ;
%Shape: Circle [id:dp15544782043727357] 
\draw  [color={rgb, 255:red, 92; green, 152; blue, 210 }  ,draw opacity=1 ][fill={rgb, 255:red, 92; green, 152; blue, 210 }  ,fill opacity=0.34 ][line width=2.25]  (386,158) .. controls (386,119.89) and (416.89,89) .. (455,89) .. controls (493.11,89) and (524,119.89) .. (524,158) .. controls (524,196.11) and (493.11,227) .. (455,227) .. controls (416.89,227) and (386,196.11) .. (386,158) -- cycle ;
%Shape: Circle [id:dp6770938271605338] 
\draw  [color={rgb, 255:red, 92; green, 152; blue, 210 }  ,draw opacity=1 ][fill={rgb, 255:red, 92; green, 152; blue, 210 }  ,fill opacity=0.34 ][line width=2.25]  (184,161) .. controls (184,122.89) and (214.89,92) .. (253,92) .. controls (291.11,92) and (322,122.89) .. (322,161) .. controls (322,199.11) and (291.11,230) .. (253,230) .. controls (214.89,230) and (184,199.11) .. (184,161) -- cycle ;
%Straight Lines [id:da27866230270828196] 
\draw    (235,240.6) -- (308.35,190.72) ;
\draw [shift={(310,189.6)}, rotate = 145.78] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


% Text Node
\draw (156, 28) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {{Space of Fisher markets}};
% Text Node
\draw (323,77) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$O\left(\nicefrac{(1+\varepsilon ^{2})}{t}\right)$};
% Text Node
\draw (325,165) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\text{Nested CES}$};
% Text Node
\draw (335,185) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$O\left(\nicefrac{1}{t}\right)$};
% Text Node
\draw (402,114) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\text{Leontief}$};
% Text Node
\draw (320,58) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\text{Homothetic}$};
% Text Node
\draw (404,129) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$O\left(\nicefrac{1}{t}\right)$};
% Text Node
\draw (482,125) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\text{WGC}$};
% Text Node
\draw (462,143) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$( 1-\Theta (1))^{t}$};
% Text Node
\draw (190,135) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\text{WGS}$};
% Text Node
\draw (188,151) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$( 1-\Theta ( 1))^{t}$};
% Text Node
\draw (193,239) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\text{CES}( \rho  >0)$};
\draw (193,255) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$( 1-\Theta ( 1))^{t}$};

\draw (453,239) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\text{CES}( \rho  <0)$};
\draw (453,255) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$( 1-\Theta (1))^{t}$};

\draw (453,240) -- (402,185) ; 

\draw [shift={(402,185))}, rotate = 42.78] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

\end{tikzpicture}
% }
   

% \end{subfigure}

==> figure2.tex <==

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da19466735661615164] 
\draw    (126,141.6) -- (479,140.6) ;
%Straight Lines [id:da8437523936437585] 
\draw    (301,8.6) -- (303,263.6) ;
%Shape: Circle [id:dp17890652043650368] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (477.4,12.6) .. controls (477.4,14.15) and (478.65,15.4) .. (480.2,15.4) .. controls (481.75,15.4) and (483,14.15) .. (483,12.6) .. controls (483,11.05) and (481.75,9.8) .. (480.2,9.8) .. controls (478.65,9.8) and (477.4,11.05) .. (477.4,12.6) -- cycle ;
%Shape: Circle [id:dp37491035792558347] 
\draw  [color={rgb, 255:red, 223; green, 82; blue, 69 }  ,draw opacity=1 ][fill={rgb, 255:red, 223; green, 82; blue, 69 }  ,fill opacity=1 ] (122.5,141.6) .. controls (122.5,143.53) and (124.07,145.1) .. (126,145.1) .. controls (127.93,145.1) and (129.5,143.53) .. (129.5,141.6) .. controls (129.5,139.67) and (127.93,138.1) .. (126,138.1) .. controls (124.07,138.1) and (122.5,139.67) .. (122.5,141.6) -- cycle ;
%Shape: Circle [id:dp0726180824745506] 
% \draw  [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (476,253.2) .. controls (476,254.75) and (477.25,256) .. (478.8,256) .. controls (480.35,256) and (481.6,254.75) .. (481.6,253.2) .. controls (481.6,251.65) and (480.35,250.4) .. (478.8,250.4) .. controls (477.25,250.4) and (476,251.65) .. (476,253.2) -- cycle ;
%Shape: Circle [id:dp4551933497851337] 
\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (299.6,126.6) .. controls (299.6,124.94) and (300.94,123.6) .. (302.6,123.6) .. controls (304.26,123.6) and (305.6,124.94) .. (305.6,126.6) .. controls (305.6,128.26) and (304.26,129.6) .. (302.6,129.6) .. controls (300.94,129.6) and (299.6,128.26) .. (299.6,126.6) -- cycle ;
%Shape: Rectangle [id:dp5157037826861641] 
\draw  [color={rgb, 255:red, 66; green, 128; blue, 183 }  ,draw opacity=0.37 ][fill={rgb, 255:red, 66; green, 128; blue, 183 }  ,fill opacity=0.35 ] (302.5,12.6) -- (478.8,12.6) -- (478.8,141.6) -- (302.5,141.6) -- cycle ;
%Shape: Rectangle [id:dp32814093651702114] 
\draw  [color={rgb, 255:red, 184; green, 133; blue, 186 }  ,draw opacity=0.35 ][fill={rgb, 255:red, 184; green, 133; blue, 186 }  ,fill opacity=0.36 ] (121,12.6) -- (302.5,12.6) -- (302.5,140.6) -- (121,140.6) -- cycle ;

% Text Node
\draw (324,-2) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Hicksian};
% Text Node
\draw (438,148) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Marshallian};
% Text Node
\draw (302.5,142) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (463,142) node [anchor=north west][inner sep=0.75pt]    {$\infty $};
% Text Node
\draw (120,142) node [anchor=north west][inner sep=0.75pt]    {$-\infty $};
% Text Node
\draw (305,255) node [anchor=north west][inner sep=0.75pt]    {$-\infty $};
% Text Node
\draw (303,3) node [anchor=north west][inner sep=0.75pt]    {$\infty $};
% Text Node
\draw (482,0) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {Linear};
% Text Node
\draw (127,121) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 223; green, 82; blue, 69 }  ,opacity=1 ] [align=left] {Leontief};
% Text Node
% \draw (484,239) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 245; green, 166; blue, 35 }  ,opacity=1 ] [align=left] {Quasilinear};
% Text Node
\draw (305,110) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ] [align=left] {Cobb-Douglas};
% Text Node
\draw (355,70) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 61; green, 124; blue, 196 }  ,opacity=1 ]  {$
\text{CES}( \rho > 0)$};
% Text Node
\draw (175,71) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 180; green, 100; blue, 203 }  ,opacity=1 ]  {$ 
 \text{CES}( \rho < 0)$};
\end{tikzpicture}
% \end{subfigure}

==> generalization.tex <==
\section{Convex Programs, Potential functions and Dynamics}
\label{sec:dynamics}

A relatively recent line of work initiated by \citeauthor{proportional-response} has aimed to analyze the convergence of various dynamics, such as proportional response and t\^atonnement, by proving the equivalence of these processes to gradient descent on a potential function \cite{proportional-response}.
In fact, \citeauthor{proportional-response} argues that an equivalence between convex programs and market dynamics arises from ``a deep mathematical structure'' \cite{proportional-response}, quoting \citeauthor{vazirani2010spending} \cite{vazirani2010spending}.
In this section, we uncover a mathematical structure that exists between potential functions and market dynamics by taking a dynamical systems approach.
Understanding this mathematical structure is important as more often than not researchers discover market dynamics that converge to equilibria before they discover the corresponding convex program.
Such was the case with t\^atonnement, which was first introduced in the 1870s by Walras \cite{walras}, even though the first convex program for the Fisher market was introduced in 1959 (and even then the relationship between the program and t\^atonnement was not recognized until the 2000s).  
A second example is the proportional response dynamics, which was first introduced by \citeauthor{first-prop-response} \cite{first-prop-response} in 2007, but whose corresponding convex program for linear utilities was not discovered until 2011 \cite{grad-prop-response} or generalized for all CES utilities until 2018 \cite{cheung2018dynamics}.

Let $\potential: \R^\numgoods \to \R$ be a convex potential function whose minima, $\argmin_{\price \in \R^\numgoods}  \potential(\price)$, capture the equilibrium prices of a market $\calM$.
For simplicity, we assume that the potential function is twice differentiable, i.e., $\potential \in \calC^{2}(\R^\numgoods)$.
We can then formulate a market dynamic based on gradient descent on the convex potential function $\potential$ as an initial value problem (IVP) given by:
%
\begin{align}
    \frac{d\price(t)}{dt} &= - \grad[\price] \potential(\price(t))\label{IVP}\\
    \price(0) &= \price^0 \in \R^{\numgoods} \label{IVP2}
\end{align}

In order to understand the behavior of the above process for any initial price vector $\price \in \R^\numgoods_+$, we define a flow $\flow: \R^{\numgoods} \times \R \to \R^\numgoods$ such that $\flow(\price, t)$ describes the price determined by the market dynamic at time $t$, given starting prices $\price$.
By convention, we denote $\flow(\price, t) = \flow[t](\price)$.
Since we assume $\potential \in C^2(\R^\numgoods)$, we also have that $\flow \in C^2(\R^\numgoods)$, and furthermore $\flow$ is a diffeomorphism.
We can thus re-express the IVP in \crefrange{IVP}{IVP2} as a continuous dynamical system with phase space $\R^{\numgoods}$ and evolution function:
%
\begin{align}
    \frac{\partial \flow}{\partial t} = - \grad[\price] \potential(\left(\flow[t](\price)\right)
\label{flow1}
\end{align}

Our goal is to understand the conditions under which a convergent market dynamic can be represented in the form of \Cref{flow1}, i.e., as gradient descent on a convex potential function, and vice versa.
%under what conditions gradient descent on a potential function corresponds to a convergent market dynamic.
To this end, we prove that a continuous-time market dynamic corresponds to gradient descent on a convex function, i.e., a process in the form of \Cref{flow1}, iff the evolution function of the system is positive semi-definite.

\begin{theorem}
\label{potential-dynamic}
Let $\calM$ be a market, e.g., a Fisher market.
There exists a twice differentiable convex potential function, $\potential: \R^\numgoods \to \R$, whose minimizers, $\argmin_{\price \in \R^\numgoods} \potential(\price)$, capture the equilibrium prices of market $\calM$ iff there exists a converging market dynamic $\frac{d\price}{dt} = f(\price(t))$ such that for all $\price \in \R^\numgoods, \grad[\price] f(\price)$ is positive semi-definite.
\end{theorem}


\begin{proof}[Proof of \Cref{potential-dynamic}]
[Potential function $\Rightarrow$ Market Dynamic]:
Let $\potential: \R^\numgoods \to \R$ be a convex potential function whose minimizers, $\argmin_{\price \in \R^\numgoods} \potential(\price)$, comprise equilibrium prices.
We define a flow $\flow: \R^{\numgoods} \times \R \to \R^\numgoods$ by:  
\begin{align}
    \frac{d}{dt} \flow[t](\price) = - \grad[\price] \potential[\price] (\flow[t](\price)) \enspace .\label{def-flow}
\end{align}
Note that since $\potential$ is convex, $\grad[\price] \potential$ is positive semi-definite.
\noindent
We claim that $\forall \price \in \R^\numgoods, \lim_{t \to \infty} \flow[t](\price) = \price^*$, for some $\price^* \in \argmin_{\price \in \R^\numgoods} \potential(\price)$.
%The proof follows similarly to the convergence proof we gave for continuous t\^atonnement.
%\amy{if this theorem generalizes that one, let's not include that proof, only this one. for that one, just say, it's a special case of this one. (same proof.)}

Define $v(t) = \potential[\price] (\flow[t](\price))$ to evaluate the distance between the prices determined at time $t$ by the market dynamic, i.e., $\price(t)$, and the equilibrium $\price^*$.
We have:
\begin{align}
    \frac{dv}{dt}
    &= \grad[\price](\potential(\flow[t](\price))) \cdot \frac{d\flow[t]}{dt} \\
    &= \grad[\price](\potential(\flow[t](\price))) \cdot - \grad[\price] \potential[\price] (\flow[t](\price)) && \text{(\Cref{def-flow})} \\
    &= - \left| \left| \grad[\price] \potential[\price] (\flow[t](\price))\right| \right|_2^2
\end{align}

\noindent
Re-expressing $v(t)$ as an integral equation, we have:
\begin{align}
    v(t) 
    &= v(0) + \int_0^t - \left| \left| \grad[\price] \potential[\price] (\flow[t](\price))\right| \right|_2^2 dt \\
    &= v(0) - \int_0^t  \left| \left| \grad[\price] \potential[\price] (\flow[t](\price))\right| \right|_2^2 dt
\end{align}

Note that $\left| \left| \grad[\price] \potential[\price] (\flow[t](\price))\right| \right|_2^2 > 0$, unless $\price(t) = \price^*$.
Hence, for any time $t > s$, we have $v(t) < v(s)$
%\amy{strict?}\deni{yes!}
unless $\price(s) = \price(t)$, i.e., the process has converged.
Since $\potential[\price]$ is convex, and its minimum exists, we must then have $\lim_{t \to \infty} \flow[t](\price) = \price^*$ for some $\price^* \in \argmin_{\price \in \R^\numgoods} \potential(\price)$.

[Market Dynamic $\Rightarrow$ Potential function]:
Suppose $\frac{d\price}{dt} = f(\flow[t](\price))$ is a market dynamic on the phase space $\R^\numgoods$ which converges for any starting point in the phase space. Define the omega limit set of a set $A \subseteq \R^\numgoods$ as $\omega(A) = \left\{\y \in \R^\numgoods \mid \exists t^{(n)} \to \infty, \price^{(n)} \in A, \text{ such that } \flow[{t^{(n)}}](\price^{(n)}) \to \y \right\}$. Let $\price^0 \in \R^\numgoods$ and $\price^* \in \omega(\{\price^0\})$. Then, by the fundamental theorem of line calculus, there exists at least one function $g$, namely the line integral of $f$ over the curve $\gamma(t) = \flow[t](\price^0)$. Additionally, if $\grad[\price]f(\price)$ is positive semi-definite, then $g$ is convex and $\price^*$ is a mimimizer.
\end{proof}

\Cref{potential-dynamic} allows us to understand the relationship between potential functions and market dynamics as well understood objects from dynamical systems theory, namely the gradient flow.
Gradient flows occur in many systems, where the potential function measures the energy left in the system, while the gradient of the potential function gives the behavior of the system across time as it is losing energy, eventually coming to a full stop. The same holds for our potential function where \Cref{potential-func} records the trade-off between the surplus of the auctioneer and that of buyers.
The potential function can be understood as an abstraction for the tensions caused by this surplus maximizing behavior on both sides of the market.
This tension is resolved, and the market can settle into equilibrium once the market forces follow the negative gradient of the potential function.
Such a view, also supports \citeauthor{cole2008fast}'s findings that t\^atonnement is an abstraction for in-market processes \cite{cole2008fast, cole2010discrete}.

% An important characteristic of a gradient flow is that for any point in the phase space, the flow is guaranteed to converge. This is very similar to how the potential function we present for Fisher markets works too. Once the t\^atonnement process is initiated, the distance from equilibrium can only go down as the Fisher market is ``running out of energy''. The gradient flow interpretation in a way confirms that t\^atonnement could be a plausible market dynamic, since it essentially says that any Fisher market that has potential energy will start moving as determined by determined by the negative of the gradient of the potential function. This is very similar to a ball rolling down hill with some initial potential energy. It is hard to understand the physical explanation that leads a ball to accumulate potential energy when on top of a hill, but the potential energy abstraction allows us to abstract out the layers of complexity existing in the real world, e.g., atoms colliding, and to predict the behavior of the system until it runs out of energy. Similarly, the potential function we formulate in this paper can be seen as an abstraction of the economic complexities existing in real markets, and the gradient of our potential function can be seen as an abstraction for the market processes that lead markets to equilibrium. 

%\amy{all of the above is true. but noticed first by Cole, or others before him. you only need one sentence here about economics solely. saying that the excess demand is the potential, and the market dynamic is decreasing that excess demand. end of story.}\deni{Ok, I know you do not want me to write more but I really like the above modified interpretation. Since our potential function is a trade-off between the consumer's surplus and the market's(or auctioneer's) surplus, it is an abstraction for the tensions within the market and these tensions get resolved once we follow the negative gradient. I think this interpretation of the potential function for Fisher markets new and adds an interesting angle to the discussion. It also supports the argument that tatonnement is an abstraction for in market processes. What do you think?}

Finally, using a proof similar to the first part of the proof of \Cref{potential-dynamic}, we can obtain the convergence of continuous-time t\^atonnement in homothetic Fisher markets, since the potential function we proposed for homothetic Fisher markets is convex.

\begin{theorem}
\label{continuous-tatonnement-convergence}
Suppose that $(\util, \budget)$ is a homothetic Fisher market with equilibrium prices $\price^*$. The asymptotic behavior of the flow in \Cref{flow1} is stable for the potential function \Cref{potential-func} and converges to the equilibrium price vector, $\price^*$, of the Fisher market corresponding to the excess demand function $\excess: \R^\numgoods \to \R^\numgoods$, i.e., $\forall \price \in \R^{\numgoods}_+, \ \  \lim_{t \to \infty} \flow[t](\price) = \price^*$.
\end{theorem}

% We note that this theorem can be easily extended to any continuous-time t\^atonnement process as given in \Crefrange{tatonnement}{tatonnement2}, by replacing the time derivative of prices with the desired t\^atonnement update rule.


==> money.tex <==
\section{Hahn's Problem} \label{sec:money}

\sdeni{}{
One of the main economic challenges in building general equilibrium models which was first posed by Frank Hahn, and to this day remains relatively unsolved, lies in constructing models in which consumers have no preference for money yet money has a non-zero value at equilibrium \cite{Hahn1989}. This problem is nowadays known as \mydef{Hahn's problem}. A detailed account of the problem's history in the economics literature can be found in the work of \citeauthor{Bridel2014Why} \cite{Bridel2014Why}. Early attempts at providing general equilibrium models that guaranteed a non-zero value for money were initiated by Don Patinkin who was able to ensure a positive equilibrium value for money \emph{albeit} by placing money inside the utility function, i.e., by making money part of the space of goods. This theoretical decision attracted much controversy as it was seen as a theoretically unwell by some of the main figure in general equilibrium theory such as Ross Starr. So much so, that in a 1990 paper, \citeauthor{starr1990money} have argued that ``putting money, even real money balances, into the utility function is an unreliable choice-theoretic short cut for modelling the transactions role of money'' \cite{starr1990money}. In this section, we will provide a mathematical perspective to this controversy in the context of Fisher markets that is distinct from the economic ones. In particular, we will show that when the space of goods includes money and consumers are able to (potentially) attribute value to money, a simpler mathematical generalization of the Eisenberg-Gale and Devanur's program are possible.

}
\subsection{A Relationship between Quasilinear Utilities and Linear Utilities}

Although our program provides a generalization of the Eisenberg-Gale program, if one computes the expenditure function associated with quasilinear utilities, one will in fact not obtain Devanur's program, \sdeni{}{and one has to first convert the program into an equivalent linear Fisher market in order to obtain Devanur's program}. 
\amy{how DO you obtain it?}
The reason for this is, quasilinear utilities are \emph{not\/} locally non-satiated, making our results inapplicable to them. However, all hope is not lost as one can transform any quasilinear utility into an equivalent locally non-satiated utility function. In particular, any quasilinear utility function can be converted into a linear utility function in which the artificial currency the buyers spend is considered as another good for which they have a value of 1. It then turns out that the Marshallian and Hicksian demands associated with this new utility function are the same as those associated with the original quasilinear utility function. We note, however, that this does not mean that both utility functions represent the same preferences since the space on which the preference relation is defined is different for the two utility functions. Our results implies that any results that apply to linear Fisher markets, which are quite well understood, also apply to quasilinear \sdeni{}{Fisher markets since any quasilinear Fisher market can be converted into a linear Fisher market with a space of goods with an additional dimension}.\amy{or Fisher markets? which is it?}\deni{Discuss}
% More generally, utility functions that attribute value to money and that are not locally non-satiated can be rendered locally non-satiated via a construction similar to that provided below.

\begin{theorem}\label{quasi-equiv-linear}
Consider a quasilinear utility function $\util[\buyer]: \R^\numgoods \times \R^\numgoods \to \R$ given by $\util[\buyer](\allocation[\buyer]; \price) = \allocation[\buyer] \cdot \left( \valuation[\buyer] - \price \right)$ and a linear utility function $\util[\buyer]^\prime: \R^{\numgoods + 1} \to \R$ given by: 
%
\begin{align}\label{equiv-util}
    \util[\buyer]^\prime(\allocation[\buyer]^\prime) =  \allocation[\buyer]^\prime \cdot  \begin{pmatrix} \valuation[\buyer] \\ 1
    \end{pmatrix}
\end{align}
The Marshallian demand at prices $\price$ and budget $\budget[\buyer]$ associated with quasilinear utility function $\util[\buyer]$ is equal to the Marshallian demand at prices $(\price, 1)^T$ and budget $\budget[\buyer]$ associated with $\util[\buyer]^\prime$. Additionally, the Hicksian demand at prices $\price$ and utility level $\goalutil[\buyer]$ associated with quasilinear utility function $\util[\buyer]$ is equal to the Hicksian demand at prices $(\price, 1)^T$ and utility level $\goalutil[\buyer]$ associated with $\util[\buyer]^\prime$. 
\end{theorem}

\begin{proof}
Before we present the proof, we first recall the optimality conditions of the Marshallian demand at prices $\price$ and budget $\budget[\buyer]$ for quasilinear utilities, and then we derive the optimality condition of the Marshallian demand for $\util[\buyer]^\prime$ at prices $\price$ and budget $\budget[\buyer]$.

The first order necessary and sufficient optimality conditions for a vector $\allocation[\buyer]^\star \in \R^\numgoods$ to be the Marshalian demand of quasilinear utilities $\util[\buyer]$ is given by:
\begin{align}
    \allocation[\buyer][\good]^\star > 0 \implies  \frac{\valuation[\buyer][\good] - \price[\good]}{\price[\good]} = \max_{k \in \goods} \frac{\valuation[\buyer][k] - \price[k]}{\price[k]}\label{quasilinear-equimarginal}
\end{align}

\noindent
That is, buyers demand a set of goods which provide them with maximal bang-per-buck $\frac{\valuation[\buyer][\good] - \price[\good]}{\price[\good]}$, and if none of the goods have a positive bang-per buck then the buyer purchases nothing and its budget is not spent.

The Marshallian demand associated with \Cref{equiv-util} at prices $(\price, 1)^T$ and budget $\budget[\buyer]$ is given by the UMP:
\begin{align}
    \max_{\allocation[\buyer]^\prime \geq 0: \allocation[\buyer]^\prime \cdot (\price, 1)^T
     \leq \budget[\buyer]} \allocation[\buyer]^\prime \cdot  \begin{pmatrix} \valuation[\buyer] \\ 1
    \end{pmatrix}
\end{align}

The Lagrangian associated with the above UMP is given by:

\begin{align}
    L(\allocation[\buyer]^\prime, \lambda, \bm{\mu}) = \allocation[\buyer]^\prime \cdot  \begin{pmatrix} \valuation[\buyer] \\ 1
    \end{pmatrix} + \lambda \left(\budget[\buyer] - \allocation[\buyer]^\prime \cdot \begin{pmatrix} \price \\ 1
    \end{pmatrix}\right) +  \bm{\mu}^T \allocation[\buyer]^\prime
\end{align}
where $(\lambda, \bm{\mu}) \in \R_+ \times \R^{\numgoods +1}$ are the Lagrangian multipliers associated with the budget and non-negativity constraints respectively.

The first order KKT stationarity condition for this Lagrangian are given by:
\begin{align}
    \grad[{\allocation[\buyer]^\prime}] L  = \begin{pmatrix} \valuation[\buyer] \\ 1
    \end{pmatrix} - \lambda \begin{pmatrix} \price \\ 1
    \end{pmatrix} + \bm{\mu} = 0
\end{align}
Re-organizing terms, we obtain:
%
\begin{align}
    \lambda = \frac{\begin{pmatrix} \valuation[\buyer] \\ 1
    \end{pmatrix}_\good - \mu_\good}{\begin{pmatrix} \price \\ 1
    \end{pmatrix}_\good}
\end{align}
If $\allocation[\buyer][\good]^\prime > 0$, by the KKT complementary slackness conditions, we have that $\mu_\good = 0$, so
\begin{align}
    \allocation[\buyer][\good]^\prime > 0 \implies \lambda =
    % \max_{\good \in [\numgoods + 1]} 
    \frac{\begin{pmatrix} \valuation[\buyer] \\ 1
    \end{pmatrix}_\good }{\begin{pmatrix} \price \\ 1
    \end{pmatrix}_\good}\label{utilprime-equimarginal}
    % \allocation[\buyer][\good]^\prime > 0 \implies \lambda = \max\left\{1, \max_{\good \in \goods}  \frac{\valuation[\buyer][\good]}{\price[\good]} \right\}
\end{align}

\paragraph{Case 1: For all goods $\good \in \goods$, $\price[\good] \geq \valuation[\buyer][\good]$}

By \Cref{quasilinear-equimarginal}, the Marshallian demand of the buyer under $\util[\buyer]$ is a convex combination of goods such that $\valuation[\buyer][\good] - \price[\good] = 0$ (up to the budget constraint) and the empty set.

By \Cref{utilprime-equimarginal}, the Marshallian demand of the buyer under $\util[\buyer]^\prime$ is a convex combination of goods such that $\valuation[\buyer][\good] - \price[\good] = 0$ which also includes $\numgoods +1$. Since good $\numgoods + 1$ is money, the consumer essentially purchased nothing when they purchased $\numgoods + 1$, hence the Marshallian demands coincide.

\paragraph{Case 2: There exists $\good \in \goods$ such that $\valuation[\buyer][\good] > \price[\good]$}
% \amy{strictly greater?}

By \Cref{quasilinear-equimarginal} the Marhshallian demand under $\util[\buyer]$ is a convex combination of goods $\argmax_{k \in \goods}   \frac{\valuation[\buyer][k] - \price[k]}{\price[k]}$ up to their budget constraint.

By \Cref{utilprime-equimarginal}, under $\util[\buyer]^\prime$ the Marshallian demand of the buyer is a convex combination of goods $\argmax_{k \in \goods}   \frac{\valuation[\buyer][k]}{\price[k]}$. Note that we have the following:
\begin{align}
  \argmax_{k \in \goods}   \frac{\valuation[\buyer][k]}{\price[k]} &= \argmax_{k \in \goods}   \frac{\valuation[\buyer][k]}{\price[k]} -1\\
  &= \argmax_{k \in \goods}   \frac{\valuation[\buyer][k] -  \price[k]}{\price[k]} 
\end{align}
Hence, the Marshallian demands coincide. The proof proceeds similarly for the Hicksian demand.
\end{proof}

\sdeni{}{The above result determines a roadmap to convert any quasilinear Fisher market into a linear Fisher market. Given a quasilinear Fisher market $(\util, \budget)$ one can convert it into a linear Fisher market $(\util^\prime, \budget)$ using the equivalence given in \Cref{quasi-equiv-linear}. One will notice then, that the expenditure functions associated with utility functions $\util^\prime$ at any price $(\price, 1)^T$ and budgets $\budget$ give exactly Devanur's program.} This equivalence can also be used to extend the results concerning algorithms solving linear Fisher markets using Marshallian and/or Hicksian demands to quasilinear Fisher markets. For instance, \citeauthor{cole2019balancing}'s results for the convergence of t\^atonnement in linear Fisher markets can be directly extended to quasilinear Fisher markets and the convergence results of the algorithms introduced by \citeauthor{gao2020first} \cite{gao2020first} for linear Fisher markets can be trivially extended to quasilinear Fisher markets.

\subsection{A simpler generalization via Extension of Space of Goods}

We define a \mydef{Patinkin utility function} as any utility function that attributes value to money. More specifically, a Patinkin utility function is a utility function whose domain is the space of goods extended to include money, i.e., $\util[\buyer]: \R^{\numgoods + 1} \to \R$. We name this class after Patinkin who was first to use utility functions which attribute value to money \cite{Hahn1989}. Patinkin utility functions treat  

%
\begin{equation*}
\begin{aligned}[c]
    &\text{\textbf{Primal}} \\ &\max_{\allocation \in \R^{\numbuyers \times \numgoods + 1}_+} & \sum_{\buyer \in \buyers} \budget[\buyer] \log{\left(\util[\buyer](\allocation[\buyer])\right)} - \allocation[\buyer,][(\numgoods + 1)] \\
    & \forall \good \in \goods & \sum_{\buyer \in \buyers} \allocation[\buyer][\good] \leq 1 \\
\end{aligned}
\quad \vline \quad
\begin{aligned}[c]
    &\text{\textbf{Dual}} \\ &\min_{\price \in \R^\numgoods_+} & \sum_{\good \in \goods} \price[\good] - \sum_{\buyer \in \buyers} \budget[\buyer] \log{\partial_{\goalutil[\buyer]}{\expend[\buyer] (\price, \goalutil[\buyer])}} 
\end{aligned}
\end{equation*}

==> overview.tex <==
\subsection{A High-Level Overview of Our Contribution}

%Our paper is centered around \samy{two}{three} main results.

In this paper, we bring consumer theory to bear in the analysis of CCH Fisher markets.
In so doing, we first derive the dual of the Eisenberg-Gale program for arbitrary CCH Fisher markets, generalizing the special cases of linear and Leontief markets, which were already understood~\cite{devanur2008market}.
We then provide a new convex program whose dual also characterizes equilibrium prices in CCH Fisher markets via expenditure functions.
This program is of interest because the subdifferential of the objective function of its dual is equal to the negative excess demand in the market, which implies that (generalized) gradient descent on this objective is equivalent to solving for equilibrium prices in the associated market via t\^atonnement.
Finally, using this equivalence, we extend the sublinear convergence rate of $O(\nicefrac{1}{t})$ known for Leontief Fisher markets to the entire class of CSCH Fisher markets.

%%% OLD, but proofread to double check none of this is needed!
\if 0
We first derive the dual of the Eisenberg-Gale program, and observe that our dual differs from that of  \citeauthor{cole2019balancing} by only a constant factor.
We then provide a convex program for CCH Fisher markets that characterizes the equilibrium prices of CCH Fisher markets via expenditure functions.
This characterization allows us to provide a new, direct computational proof that the subgradient of the objective function of the dual is equal to the excess demand, a fact previously proven by \citeauthor{fisher-tatonnement} \cite{fisher-tatonnement} via an indirect Lagrangian argument.\amy{delete!}
It also allows us to generalize \citeauthor{fisher-tatonnement}'s \cite{fisher-tatonnement} proof of the convergence of t\^atonnement in CES Fisher markets to all CSCH Fisher markets (\Cref{sec:convergence}).
\fi

Although the Eisenberg-Gale convex program dates back to 1959, its dual for arbitrary CCH Fisher markets is still not yet well understood.
Our first result is to derive the Eisenberg-Gale program's dual, generalizing the two special cases identified by \citeauthor{cole2016convex} \cite{cole2016convex} for linear and Leontief utilities.
% Studying the Eisenberg-Gale program via the well-understood building blocks of consumer theory, e.g., UMP and EMP, gives us an intuitive understanding of its dual...

\begin{theorem}
\label{thm1-overview}
The dual of the Eisenberg-Gale program for any CCH Fisher market $(\util, \budget)$ is given by:
\begin{align}
    \min_{\price \in \R^\numgoods_+} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left[ \budget[\buyer] \log{ \left( \indirectutil[\buyer](\price, \budget[\buyer]) \right)} - \budget[\buyer] \right] \label{dual-program}
\end{align}
\end{theorem}

We then propose a new convex program whose dual characterizes the equilibrium prices of CCH Fisher markets via expenditure functions.
We note that the optimal value of this convex program differs from the optimal value of the Eisenberg-Gale program by a constant factor.

\begin{theorem}
\label{thm2-overview}
% \label{new-convex}
The optimal solution $(\allocation^*, \price^*)$ to the primal and dual of the following convex programs corresponds to equilibrium allocations and prices, respectively, of the CCH Fisher market $(\util, \budget)$:
\begin{equation*}
\begin{aligned}[c]
    &\text{\textbf{Primal}} \\  
    & \max_{\allocation \in \R_+^{\numbuyers \times \numgoods}} & \sum_{\buyer \in \buyers} 
    % \left[ 
    \budget[\buyer] \log{\left(\util[\buyer]\left(\frac{\allocation[\buyer]}{\budget[\buyer]}\right)\right)} 
    % + \budget[\buyer] \right] 
    \\
    & \text{subject to} & \sum_{\buyer \in \buyers} \allocation[\buyer][\good] & \leq 1 &&\forall \good \in \goods\\
    % && \allocation[\buyer][\good] &\geq 0 &&\forall \buyer \in \buyers, \good \in \goods 
\end{aligned}
\quad \vline \quad
\begin{aligned}[c]
    &\text{\textbf{Dual}} \\  &\min_{\price \in \R^\numgoods_+} \sum_{\good \in \goods} \price[\good] - \sum_{\buyer \in \buyers} \budget[\buyer] \log{ \left( \partial_{\goalutil[\buyer]}{\expend[\buyer] (\price, \goalutil[\buyer])} \right)}
\end{aligned}
\end{equation*}
\end{theorem}

This convex program formulation for CCH Fisher markets is of particular interest because its subdifferential equals the negative excess demand in the market.
As a result, solving this program via (sub)gradient descent is equivalent to solving the market via t\^atonnement. 

\begin{theorem}
\label{thm3-overview}
The subdifferential of the objective function of the dual of the program given in \Cref{thm2-overview} for a CCH Fisher market $(\util, \budget)$ at any price $\price$ is equal to the negative excess demand in $(\util, \budget)$ at price $\price$:
%
\begin{align}   
    \subdiff[\price] \left( \sum_{\good \in \goods} \price[\good] - \sum_{\buyer \in \buyers} \budget[\buyer] \log{ \partial_{\goalutil[\buyer]}{\expend[\buyer] (\price, \goalutil[\buyer])}} \right) %= \bm{1}_{\numgoods} - \sum_{\buyer \in \buyers} \marshallian[\buyer](\price, \budget[\buyer])  
    = - \excess(\price)
\end{align}
\end{theorem}

To prove \Cref{thm3-overview}, we make use of standard consumer theory, specifically the duality structure between UMP and EMP, as well as a generalized version of Shepherd's lemma \cite{shephard, generalized-shephard}.
We also provide a new, simpler proof of this generalization of Shepherd's lemma via Danskin's theorem \cite{danskin1966thm}.

Our fourth result concerns the convergence of the t\^atonnement process defined by the generalized gradient descent rule with KL-divergence and fixed step sizes
%given in \Crefrange{generalized-descent}{generalized-descent2}
in CSCH Fisher markets.
This particular t\^atonnement rule was previously studied by \citeauthor{fisher-tatonnement} \cite{fisher-tatonnement} in Leontief Fisher markets.
Our result extends the sublinear convergence rate of $O(\nicefrac{1}{t})$ they obtained for Leontief Fisher markets to the entire class of CSCH Fisher markets, which includes classes of markets for which convergence results were not previously known, such as mixed and nested CES markets \cite{cheung2018dynamics, jain2006equilibria}.
We note that it is our novel characterization of equilibrium prices via expenditure functions that allows us to generalize \citeauthor{fisher-tatonnement}'s \cite{fisher-tatonnement} convergence result to all CSCH Fisher markets.

\begin{theorem}
\label{thm4-overview}
Let $f(\price) = \sum_{\good \in \goods} \price[\good] - \sum_{\buyer \in \buyers} \budget[\buyer] \log{ \left( \partderiv[{\expend[\buyer] (\price, \goalutil[\buyer])}][{\goalutil[\buyer]}] \right)}$. The following holds for the t\^atonnement process
%given in \Crefrange{tatonnement}{tatonnement2}
when run on a CSCH Fisher market $(\util, \budget)$:
%\begin{align}
$f(\price(t)) - f(\price^*) \leq \nicefrac{1}{t} \left( \gamma \divergence[\mathrm{h}][\price^*][\price(0)] \right)$,
%\enspace ,
%\end{align}
where $\gamma = 5 \max_{\substack{\good \in \goods\\ t \in \N}} \left\{\sum_{\buyer \in \buyers}\marshallian[\buyer][\good]\left(\price(t), \budget[\buyer]\right) \right\}$.
% 10 \cdot \max_{\good \in \goods} \left\{ \left[ \frac{\sum_{\buyer \in \buyers} \budget[\buyer]}{\price[\good]^0} \max \left\{\max_{k \in \goods}\demand[k]^0,  \frac{\max_{l \in \goods}\demand[l]^0}{\demand[\good]^0} \right\} + \max_{k \in \goods} \frac{\demand[\good]^0}{  \demand[k]^0} \right] \right\}$ and $\divergence[\mathrm{h}] = 6 \cdot \divergence[\mathrm{KL}][][]
\end{theorem}

\noindent
We provide an upper bound on $\gamma$ for mixed CCH Fisher markets
% \amy{why not call this $\gamma$? or $\gamma/5$, if you prefer?} $\max_{\substack{\good \in \goods\\ t \in \N}} \left\{\sum_{\buyer \in \buyers}\marshallian[\buyer][\good]\left(\price(t), \budget[\buyer]\right) \right\}$ 
in \Cref{sec:equiv}, so that the step size can be set when the process is initialized.
For other markets, we provide a naive upper bound when the number of iterations for which t\^atonnement will be run in known in advance, which can then be combined with the doubling trick 
% \cite{hazan2014doubling}\amy{why this particular reference?}\deni{Seemed like the thing to cite but I am clearly wrong!}\amy{the doubling trick is VERY old. i am not sure what to cite actually. but maybe nothing?}\deni{Ok, i guess it is common knowledge then!}
so that the convergence bound holds for t\^atonnement run without a known time horizon.
We note that our convergence bounds can be improved by a constant factor in future work that derives tighter bounds on the demand, since 
%the learning rate 
$\gamma$ is a function of the demand.

% \sdeni{At a high level, our approach follows the approach taken by  \citeauthor{fisher-tatonnement} \cite{fisher-tatonnement}. First, we prove a lemma that states assumptions under which the condition of \Cref{theorem-devanur} holds when $f(\price) = \sum_{\good \in \goods} \price[\good] - \sum_{\buyer \in \buyers} \budget[\buyer] \log{ \left( \partderiv[{\expend[\buyer] (\price, \goalutil[\buyer])}][{\goalutil[\buyer]}] \right)}$. For these assumptions to hold, we require that the learning rate $\gamma$ be five times the maximum demand for any good throughout the t\^atonnment process. In order to set $\gamma$ at the beginning of t\^atonnement, we upper bound this maximum demand. Once this bound is derived, we apply \Cref{theorem-devanur} to obtain the convergence rate of $O(\nicefrac{1}{t})$.}{}


==> program.tex <==
\section{The Dual of the Eisenberg-Gale Program}
\label{sec:EG-dual}

For CCH Fisher markets, the Eisenberg-Gale program's primal allows us to calculate the equilibrium allocations, while its dual yields the corresponding equilibrium prices \cite{chen2007note}.
%\deni{Even if the dual was not known, we know the dual gives equilibrium prices because the slack variables corresponding to the allocation constraints are interpreted as prices in the proof of optimality of the EG program for Fisher markets equilibria. Since the slack variables become the variables in the dual, even if we do not know the dual, we know that the prices are the decision variables in the dual!}
\citeauthor{cole2016convex} \cite{cole2016convex} provide dual formulations of the Eisenberg-Gale program for linear and Leontief utilities \cite{cole2016convex}, and in unpublished work, \citeauthor{cole2019balancing} \cite{cole2019balancing} present a generalization of the Eisenberg-Gale dual for arbitrary CCH utility functions. However, as we show in \Cref{dual-diff-cole} (\Cref{sec:Proofs3}), the optimal value of the objective of the Eisenberg-Gale program's primal differs from the optimal value of the dual provided by \citeauthor{cole2019balancing} \cite{cole2019balancing} by a constant factor, despite their dual characterizing equilibrium prices accurately.
%\amy{do you want to double check that they haven't updated their paper recently?}\deni{Not updated!}
Hence, their dual is technically not the dual of the Eisenberg-Gale program for which strong duality holds.
%\amy{let's just please be very careful not to be insulting.}

%Our dual differs from that of  \citeauthor{cole2019balancing} by only a constant factor, namely the sum of the buyers' budgets \sdeni{}{which implies that loosely speaking both programs are equivalent}.

%\amy{i think it only makes sense to include this example if we also provide their dual in the preliminary section. we don't have to do it in the two column format, since it is not the dual of EG. but if we want to talk about it at all, we do need to say what it is. another idea is to just present their dual and this counterexample in an appendix. that also works fine.}

We now derive the dual of the Eisenberg-Gale program.
We begin with an essential lemma, which states that UMP for CCH utility functions can be expressed as an unconstrained optimization problem.
A proof of this lemma can be found in \Cref{sec:Proofs3}. 

\begin{restatable}{lemma}{equivoptim}
\label{equiv-optim}
The optimization problem
\begin{align}
\max_{\allocation[\buyer] \in \R^\numgoods_+: \allocation[\buyer] \cdot \price \leq \budget[\buyer]} \budget[\buyer] \log (\util[\buyer](\allocation[\buyer]))
\end{align}
is equivalent to the optimization problem
\begin{align}
    \max_{\allocation[\buyer] \in \R_+^\numgoods} \left\{\budget[\buyer] \log(\util[\buyer](\allocation[\buyer])) + \budget[\buyer] - \allocation[\buyer] \cdot \price \right\}
\enspace .
\end{align}
\end{restatable}

With this lemma in hand, we can now derive the dual of the Eisenberg-Gale program.

\begin{theorem}
\label{EG-generalization}
The dual of the Eisenberg-Gale program for any CCH Fisher market $(\util, \budget)$ is given by
%
\begin{align}
    \min_{\price \in \R^\numgoods_+} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left( \budget[\buyer] \log{ \left( \indirectutil[\buyer](\price, \budget[\buyer]) \right)} - \budget[\buyer] \right) \enspace .
    \label{convex-program1}
    %\label{eg-dual}
\end{align}
\end{theorem}

\begin{proof}
The Lagrangian dual function $g: \R^\numgoods \to \R$ of the Eisenberg-Gale primal is given by:
%
\begin{align*}
    g(\price) 
    &= \max_{\allocation \in \R^{\numbuyers \times \numgoods}_+} L(\allocation, \price) \\
    &= \max_{\allocation \in \R^{\numbuyers \times \numgoods}_+} \left\{ \sum_{\buyer \in \buyers} \budget[\buyer] \log( \util[\buyer] (\allocation[\buyer])) + \sum_{\good \in \goods} \price[\good] \left( 1 - \sum_{\buyer \in \buyers} \allocation[\buyer][\good] \right) \right\} \\
    %&= \sum_{\good \in \goods} \price[\good] + \max_{\allocation \in \R^{\numbuyers \times \numgoods}_+} \left\{ \sum_{\buyer \in \buyers} \budget[\buyer] \log( \util[\buyer] (\allocation[\buyer])) - \sum_{\good \in \goods} \sum_{\buyer \in \buyers} \price[\good] \allocation[\buyer][\good] \right\} \\
    &= \sum_{\good \in \goods} \price[\good] +  \max_{\allocation \in \R^{\numbuyers \times \numgoods}_+} \left\{ \sum_{\buyer \in \buyers} \left( \budget[\buyer] \log( \util[\buyer] (\allocation[\buyer])) - \sum_{\good \in \goods} \price[\good] \allocation[\buyer][\good] \right)\right\} \\
    &= \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \max_{\allocation[\buyer] \in \R^{ \numgoods}_+} \left\{\budget[\buyer] \log(\util[\buyer] (\allocation[\buyer])) - \sum_{\good \in \goods} \price[\good] \allocation[\buyer][\good] \right\} \\
    %&= \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \max_{\allocation \in \R^{\numbuyers \times \numgoods}_+} \left\{ \budget[\buyer] \log( \util[\buyer] (\allocation[\buyer])) + \budget[\buyer] - \budget[\buyer] - \price \cdot \allocation[\buyer] \right\} \\
    &= \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left[ \max_{\allocation[\buyer] \in \R^{ \numgoods}_+} \left\{ \budget[\buyer] \log( \util[\buyer] (\allocation[\buyer])) + \budget[\buyer] - \price \cdot \allocation[\buyer] \right\} - \budget[\buyer] \right] \\
    &= \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left[ \max_{\allocation[\buyer] \in \R^\numgoods_+: \allocation[\buyer] \cdot \price \leq \budget[\buyer]} \budget[\buyer] \log (\util[\buyer] (\allocation[\buyer])) - \budget[\buyer]\right] && \text{(\Cref{equiv-optim})} \\
    &= \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left[ \budget[\buyer] \log \left(\max_{\allocation[\buyer] \in \R^\numgoods_+: \allocation[\buyer] \cdot \price \leq \budget[\buyer]} \util[\buyer](\allocation[\buyer]) \right) - \budget[\buyer]\right] \\
    &= \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left( \budget[\buyer] \log \left( \indirectutil[\buyer] (\price, \budget[\buyer]) \right) - \budget[\buyer] \right)
\end{align*}

\noindent
The order of the $\max$ and the sum over all buyers can be interchanged in this proof because prices are given, which renders the maximization problem for buyer $\buyer$ independent of that of buyer $\buyer'$.

Therefore, the Eisenberg-Gale dual is $\min_{\price \in \R^\numgoods_+} g(\price) = \min_{\price \in \R^\numgoods_+} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left( \budget[\buyer] \log \left(\indirectutil[\buyer](\price, \budget[\buyer])\right) - \budget[\buyer] \right)$.
\end{proof}


\section{A New Convex Program for CCH Fisher Markets}\label{sec:program}

In this section, we provide an alternative convex program to the Eisenberg-Gale program, which also characterizes the equilibria of CCH Fisher markets.
Of note, our program characterizes equilibrium prices via expenditure functions.
%
Before presenting our program, we present several preliminary lemmas.

\begin{lemma}
\label{homo-expend}
\label{homo-indirect-util}
Suppose that $\util[\buyer]$ is homogeneous, i.e., $\forall \lambda > 0, \util[\buyer](\lambda \allocation[\buyer]) = \lambda \util[\buyer]( \allocation[\buyer])$.
Then, the expenditure function and the Hicksian demand are homogeneous in $\goalutil[\buyer]$, i.e., for all $\forall \lambda > 0$, $ \expend[\buyer](\price, \lambda \goalutil[\buyer]) = \lambda \expend[\buyer](\price,  \goalutil[\buyer])$ and $\hicksian[\buyer](\price, \lambda \goalutil[\buyer]) = \lambda \hicksian[\buyer](\price, \goalutil[\buyer])$.
Likewise, the indirect utility function and the Marshallian demand are homogeneous in $\budget[\buyer]$, i.e., for all $\forall \lambda > 0$, $\indirectutil[\buyer](\price, \lambda \budget[\buyer]) = \lambda \indirectutil[\buyer](\price, \budget[\buyer])$ and $\marshallian[\buyer](\price, \lambda \budget[\buyer]) = \lambda \marshallian[\buyer](\price, \budget[\buyer])$.
\end{lemma}

\begin{proof}
%[Proof of \Cref{homo-expend}]
Without loss of generality, assume $\util[\buyer]$ is homogeneous of degree 1.%
\footnote{If the utility function is homogeneous of degree $k$, we can use a monotonic transformation, namely take the $k^{th}$ root, to transform the utility function into one of degree 1, while still preserving the preferences that it represents.}

For Hicksian demand, we have that:
\begin{align*}
    \hicksian[\buyer](\price, \lambda \goalutil[\buyer]) 
    = \argmin_{\allocation[\buyer]: \util[\buyer](\allocation[\buyer]) \geq \lambda \goalutil[\buyer]} \price \cdot \left(\lambda \frac{\allocation[\buyer]}{\lambda} \right) 
    = \lambda \argmin_{\allocation[\buyer]:  \util[\buyer](\frac{\allocation[\buyer]}{\lambda} ) \geq \goalutil[\buyer]} \price \cdot \left( \frac{\allocation[\buyer]}{\lambda} \right) = \argmin_{\allocation[\buyer]: \util[\buyer] \left(\allocation[\buyer] \right) \geq \goalutil[\buyer]} \price \cdot \allocation[\buyer] 
    = \lambda \hicksian[\buyer](\price, \goalutil[\buyer]) \enspace . \label{eq:homo-expend}
\end{align*}

\noindent 
The first equality follows from the definition of Hicksian demand;
the second, by the homogeneity of $\util[\buyer]$;
the third, by the nature of constrained optimization; and the last, from the definition of Hicksian demand again. 
% Substituting $\bm{\chi_{\buyer}} = \frac{1}{\lambda} \allocation[\buyer]$, we obtain the homogeneity of Hicksian demand:
% \begin{align}
%     \hicksian[\buyer](\price, \lambda \goalutil[\buyer]) = \argmin_{\bm \chi_{\buyer}: \util[\buyer](\bm \chi_{\buyer}) \geq \goalutil[\buyer]} \price \cdot \lambda \bm \chi_{\buyer} 
%     = \lambda \argmin_{\bm \chi_{\buyer}: \util[\buyer](\chi_{\buyer}) \geq \goalutil[\buyer]} \price \cdot \bm \chi_{\buyer}
%     = \lambda \hicksian[\buyer](\price, \goalutil[\buyer]) \label{eq:homo-expend}
% \end{align}
%
% \noindent
% where the last equality follows from the definition of the Hicksian demand.
This result implies homogeneity of the expenditure function in $\goalutil[\buyer]$:
\begin{align*}
    \expend[\buyer](\price, \lambda \goalutil[\buyer]) = \hicksian[\buyer](\price, \lambda \goalutil[\buyer]) \cdot \price 
    = \lambda \hicksian[\buyer](\price, \goalutil[\buyer]) \cdot \price 
    = \lambda \expend[\buyer](\price, \goalutil[\buyer]) \enspace .
\end{align*}

\noindent
The first and last equalities follow from the definition of the expenditure function, while the second equality follows from the homogeneity of Hicksian demand (\Cref{eq:homo-expend}).

The proof in the case of Marshallian demand and the indirect utility function is analogous.
\if 0
Similarly, for Marshallian demand, we have:
\begin{align}
    \marshallian[\buyer] (\price, \lambda \budget[\buyer])
    &= \argmax_{\allocation[\buyer]: \price \cdot \allocation[\buyer] \leq \lambda \budget[\buyer]} \util[\buyer] \left( \lambda \left( \frac{\allocation[\buyer]}{\lambda} \right) \right)
    = \lambda \argmax_{\allocation[\buyer]: \price \cdot \left( \frac{\allocation[\buyer]}{\lambda} \right) \leq \budget[\buyer]} \util[\buyer] \left( \frac{\allocation[\buyer]}{\lambda} \right)
    %\text{(Homogeneity of $\util[\buyer]$)
    = \lambda \argmax_{\allocation[\buyer]: \price \cdot \allocation[\buyer] \leq \budget[\buyer]} \util[\buyer] (\allocation[\buyer])
    = \lambda \marshallian[\buyer](\price, \budget[\buyer]) \enspace ,
\label{eq:homo-marshallian}
\end{align}
%
\noindent
The first equality follows from the definition of Marshallian demand,
the second, from the homogeneity of $\util[\buyer]$,
the third, from a straightforward property of constrained optimization, and the last, from the definition of Marshallian demand.

This result implies homogeneity of the indirect utility function in $\budget[\buyer]$:
\begin{align}
    \indirectutil[\buyer] (\price, \lambda \budget[\buyer]) = \util[\buyer] (\marshallian[\buyer] (\price, \lambda \budget[\buyer]))
    = \util[\buyer] (\lambda\marshallian[\buyer] (\price, \budget[\buyer])) 
    = \lambda \util[\buyer] (\marshallian[\buyer] (\price,  \budget[\buyer])) 
    = \indirectutil[\buyer] (\price, \lambda \budget[\buyer]) \enspace .
\end{align}
%
\noindent
The first and last equality follow from the definition of the indirect utility function,
the second equality, from the homogeneity of Marshallian demand \Cref{eq:homo-marshallian},
and the third equality, from the homogeneity of $\util[\buyer]$.
\fi
\end{proof}

The next lemma establishes an important property of the indirect utility and expenditure functions in CCH Fisher markets that we heavily exploit in this work, namely that the derivative of the indirect utility function with respect to $\budget[\buyer]$---the bang-per-buck---is constant across all budget levels.
Likewise, the derivative of the expenditure function with respect to $\goalutil[\buyer]$---the buck-per-bang---is constant across all utility levels.
In other words, both functions effectively depend only on prices.
Not only are the bang-per-buck and the buck-per-bang constant, they equal $\indirectutil[\buyer](\price, 1)$ and $\expend[\buyer](\price, 1)$, respectively, namely their values at exactly one unit of budget and one unit of (indirect) utility.

%\amy{what do you think of using the terms cost and benefit?}\deni{I prefer cost and utility, I've seen utility of one unit of budget used in other works in the past.}\amy{i prefer benefit, since utility is overloaded. it is like cost, instead of budget or price. but on the flip side, we have utility, and values, and then utility again.}

An important consequence of this lemma is that, by picking prices that maximize a buyer's bang-per-buck, we not only maximize their bang-per-buck at all budget levels, but we further maximize their total indirect utility, given their \emph{known\/} budget.
In particular, given prices $\price^*$ that maximize a buyer's bang-per-buck at budget level 1, $\indirectutil[\buyer](\price^*, 1)$, we can easily calculate the buyer's total (indirect) utility at budget $\budget[\buyer]$ by simply multiplying $\budget[\buyer]$ by their bang-per-buck: i.e., $\indirectutil[\buyer](\price^*, \budget[\buyer]) = \budget[\buyer] \indirectutil[\buyer](\price^*, 1)$.
Here, we see quite explicitly the homogeneity assumption at work.

Analogously, by picking prices that maximize a buyer's buck-per-bang, we not only maximize their buck-per-bang at all utility levels, but we further maximize the buyer's total expenditure, given their \emph{unknown\/} optimal utility level.
In particular, given prices $\price^*$ that minimize a buyer's buck-per-bang at utility level 1, $\expend[\buyer](\price^*, 1)$,
we can easily calculate the buyer's total expenditure at utility level $\goalutil[\buyer]$ by simply multiplying $\goalutil[\buyer]$ by their buck-per-bang: i.e., $\expend[\buyer](\price^*, \goalutil[\buyer]) = \goalutil[\buyer] \expend[\buyer](\price^*, 1)$.
%Again, we see quite explicitly the homogeneity assumption at work.
Thus, solving for optimal prices at any budget level, or analogously at any utility level, requires only a single optimization, in which we solve for optimal prices at budget level, or utility level, 1.

\if 0
\deni{I am now thinking that this previous sentence plus the ones up to the lemma should be deleted. What you are saying is right, it is not a consequence of the previous lemma, rather it is a consequence of \Cref{general-indirect-expend-rel} and \Cref{inverse-expend}. I elaborated this fact in more detail there.}\amy{i deleted the one sentence. is there more to delete (or move) above?}

\amy{If we had the primal, then wouldn't we then have this?!!?}
\deni{Yes! I think that is why we do not have a budget constraint in the primal!}
By maximizing the utility of one unit of budget, we would thereby maximize the bang-per-buck at \emph{all\/} budget levels, which would then enable us to compute buyers' equilibrium utilities without knowing their expenditures at equilibrium.
\fi 

\begin{lemma}
\label{derive-expend}
\label{deriv-indirect-util}
If $\util[\buyer]$ is continuous and homogeneous of degree 1, then $\indirectutil[\buyer](\price, \budget[\buyer])$ and
$\expend[\buyer](\price, \goalutil[\buyer])$ are differentiable in $\budget[\buyer]$ and $\goalutil[\buyer]$, resp.
Further, $\subdiff[{\budget[\buyer]}] \indirectutil[\buyer](\price, \budget[\buyer]) = \left\{\indirectutil[\buyer](\price, 1) \right\}$ and
$\subdiff[{\goalutil[\buyer]}] \expend[\buyer](\price, \goalutil[\buyer]) = \left\{\expend[\buyer](\price, 1) \right\}$.

% \enr{I don't think you can pull out $(v_i + h)$ from $e_i$ as the number 1 is the constant but $(v_i + h)$ is variable. You could pull out the 1, which is not what you are doing (pulling out the 1 does not really help). Or, it could be that I am confused as to what is playing the role of the constant $\lambda$ and what is variable. Right now, I think you are thinking of $(v_i + h)$ as playing the role of the constant $\lambda$ but I don't think that works.}
% \deni{What I am doing is actually assuming something weaker than homogeneity\enr{If you are assuming something else than what is currently stated in the lemma, please update the lemma statement or else we run the risk of confusing the reader}. That is I am assuming ``homogeneity only for $x=1$`` which is weaker than assuming it for all x. A clearer way you can think about this is the following. Let $g(x) = \expend[\buyer](\price, x(v_i + h))$. By homogeneity\enr{of what? what is variable and what is a constant? I guess this is what I don't understand b/c when I read homogeneous, I am thinking of a variable and a constant, and you can pull out the constant. Maybe this is the wrong way to think about it!}, I have $g(x) = \expend[\buyer](\price, x(v_i + h)) = \expend[\buyer](\price, x)(v_i + h)$. Finally setting $x=1$, I obtain $\expend[\buyer](\price, (v_i + h)) = \expend[\buyer](\price, 1)(v_i + h)$. I had also asked this on math stack exchange after you made the same point a while ago, you can find the page \href{https://math.stackexchange.com/questions/3803281/homogeneous-function-exchange-of-variable}{here}.\enr{Ok, I see the stack exchange, I think I am sort of getting it...}}
\end{lemma}

\begin{proof}
%[Proof of \Cref{deriv-indirect-util}]
We prove differentiability from first principles: 
%
\begin{align*}
    \lim_{h \to 0} \frac{\expend[\buyer](\price, \goalutil[\buyer]+h) - \expend[\buyer](\price, \goalutil[\buyer])}{h} &= \lim_{h \to 0} \frac{\expend[\buyer](\price, (1)(\goalutil[\buyer]+h)) - \expend[\buyer](\price, (1)\goalutil[\buyer])}{h} \\
    &= \lim_{h \to 0} \frac{\expend[\buyer](\price, 1)(\goalutil[\buyer] + h) - \expend[\buyer](\price, 1)(\goalutil[\buyer])}{h} \\
    &= \lim_{h \to 0} \frac{\expend[\buyer](\price, 1)(\goalutil[\buyer] + h - \goalutil[\buyer])}{h} \\
    &= \lim_{h \to 0} \frac{\expend[\buyer](\price, 1)(h)}{h} \\
    &= \expend[\buyer](\price, 1)
\end{align*}

\noindent
The first line follows from the definition of the derivative; the second line, by homogeneity of the expenditure function (\Cref{homo-expend}), since $\util[\buyer]$ is homogeneous; and the final line follows from the properties of limits.
The other two lines follow by simple algebra.

Hence, as $\expend[\buyer](\price, \goalutil[\buyer])$ is differentiable in $\goalutil[\buyer]$, its subdifferential is a singleton with $\subdiff[{\goalutil[\buyer]}] \expend[\buyer](\price, \goalutil[\buyer]) = \left\{\expend[\buyer](\price, 1) \right\}$.
The proof of the analogous result for the indirect utility function's derivative with respect to $\budget[\buyer]$ is similar .
\end{proof}

 
%It turns out that the Hicksian demand and the expenditure function are not only related through the expenditure minimization problem (EMP).


The next lemma provides further insight into why CCH Fisher markets are easier to solve than non-CCH Fisher markets.
%For CCH utility functions,
The lemma states that the bang-per-buck, i.e., the marginal utility
%\amy{benefit?}
of an additional unit of budget, is equal to the inverse of its buck-per-bang, i.e., the marginal cost of an additional unit of utility.
Consequently, by setting prices so as to minimize the buck-per-bang of buyers, we can also maximize their bang-per-buck.
%, which by \Cref{deriv-indirect-util} also maximizes each buyer's utility constrained by their budget.
Since the buck-per-bang is a function of prices only, and not of prices and allocations together, this lemma effectively decouples the calculation of equilibrium prices from the calculation of equilibrium allocations, which
%The fact that the optimization of prices can be decoupled from allocation computation, as implied by this lemma, 
greatly simplifies the problem of computing equilibria in CCH Fisher markets.

% \deni{Combine Lemma 3 and corollary 1 and ensure to the fact the expenditure}

% \begin{lemma}
% \label{general-indirect-expend-rel}
% If buyer $\buyer$'s utility function $\util[\buyer]$ is CCH,
% %Let $\expend[\buyer](\price, \goalutil[\buyer])$ be the expenditure function of buyer $\buyer$ and $\indirectutil[\buyer](\price, \budget[\buyer])$ be the indirect utility function of buyer $\buyer$. 
% then $\subdiff[{\goalutil[\buyer]}] \expend[\buyer](\price, \goalutil[\buyer]) \cdot \subdiff[{\budget[\buyer]}] \indirectutil[\buyer](\price, \budget[\buyer]) = \{1\}$.
% \end{lemma}

\begin{lemma}
\label{inverse-expend}
If buyer $\buyer$'s utility function $\util[\buyer]$ is CCH,
%Let $\expend[\buyer](\price, \goalutil[\buyer])$ be the expenditure function of buyer $\buyer$ and $\indirectutil[\buyer](\price, \budget[\buyer])$ be the indirect utility function of buyer $\buyer$.
then
\begin{align}
    \frac{1}{\expend[\buyer](\price, 1)} = \frac{1}{\partderiv[{\expend[\buyer](\price, \goalutil[\buyer])}][{\goalutil[\buyer]}]} = \partderiv[{\indirectutil[\buyer](\price, \budget[\buyer])}][{\budget[\buyer]}] = \indirectutil[\buyer](\price, 1)
    \enspace .
\end{align}
%\amy{is $\partderiv[{\indirectutil[\buyer](\price, \budget[\buyer])}][{\budget[\buyer]}]$ well defined? why isn't this a set? likewise for the expenditure function?}\deni{$\partderiv[{\indirectutil[\buyer](\price, \budget[\buyer])}][{\budget[\buyer]}] = \indirectutil[\buyer](\price, 1)$ and $\indirectutil[\buyer](\price, 1)$ is the minimum (not minimizer) of an optimization problem, hence, it can only be unique, i.e., it is not set valued. Same for the expenditure function.}
\end{lemma}

\begin{proof}
%[Proof of \Cref{general-indirect-expend-rel}]
By \Cref{derive-expend}, we know that $\expend[\buyer](\price, \goalutil[\buyer])$ is differentiable in $\goalutil[\buyer]$ and that $\subdiff[{\goalutil[\buyer]}] \expend[\buyer](\price, \goalutil[\buyer]) = \left\{ \expend[\buyer](\price, 1) \right\}$. Similarly, by \Cref{deriv-indirect-util}, we know that $\subdiff[{\budget[\buyer]}] \indirectutil[\buyer](\price, \budget[\buyer])$ is differentiable in $\budget[\buyer]$ and that $\subdiff[{\budget[\buyer]}] \indirectutil[\buyer](\price, \budget[\buyer]) = \left\{ \indirectutil[\buyer](\price, 1) \right\}$. Combining these facts yields:
%
\begin{align*}
    \subdiff[{\goalutil[\buyer]}] \expend[\buyer](\price, \goalutil[\buyer]) \cdot \subdiff[{\budget[\buyer]}] \indirectutil[\buyer](\price, \budget[\buyer]) &=  \expend[\buyer](\price, 1) \cdot  \indirectutil[\buyer](\price, 1)  && \text{(\Cref{deriv-indirect-util})} \\
    % &=  \expend[\buyer](\price, 1) \indirectutil[\buyer](\price, 1)\\
    &= \expend[\buyer](\price, \indirectutil[\buyer](\price, 1))  && \text{(\Cref{homo-expend})} \\
    &=  1  && \text{(\Cref{expend-to-budget})}
\end{align*}

\noindent
Therefore, $\frac{1}{\partderiv[{\expend[\buyer](\price, \goalutil[\buyer])}][{\goalutil[\buyer]}]} = \partderiv[{\indirectutil[\buyer](\price, \budget[\buyer])}][{\budget[\buyer]}]$. Combining this conclusion with \Cref{deriv-indirect-util}, we obtain the result.
\end{proof}

% The fact that for CCH utilities the Marshallian consumer surplus obtained by buyer $\buyer$ due to obtaining a good can be written as $ \budget[\buyer] \log \left(\partderiv[{\expend[\buyer](\price, \goalutil[\buyer])}][{\goalutil[\buyer]}] \right)$ follows easily from an extension of the definition of Marshallian consumer surplus to markets with multiple good and the fundamental theorem of calculus. Let $\mathrm{MCS}_{\buyer}: \R^{\numgoods} \times \R^{\numgoods} \to \R$ be the Marshallian consumer surplus due to a change in prices from $\price^0$ to $\price^1$ defined as $\mathrm{MCS}_{\buyer}(\price^0, \price^1) = \int_{\price[1]^0}^{\price[1]^1} \hdots \int_{\price[\numgoods]^0}^{\price[\numgoods]^1} \marshallian[\buyer](\price, \budget[\buyer]) d\price[\numgoods] \hdots d\price[1]$. Then, for CCH utilities the consumer surplus from $\price^0 = \bm{0}$, i.e., before trade, to $\price^1 = \price$, i.e., after trade, can be written as:

% \begin{align}
%     \mathrm{MCS}_{\buyer}(\bm{0}, \price) =  \int_{\price[1]^0}^{\price[1]^1} \hdots \int_{\price[\numgoods]^0}^{\price[\numgoods]^1} \marshallian[\buyer](\price, \budget[\buyer]) d\price[\numgoods] \hdots d\price[1]
% \end{align}

We can now present our characterization of the dual of the Eisenberg-Gale program via expenditure functions.
While \citeauthor{devanur2016new} \cite{devanur2016new} provided a method to construct a similar program to that given in \Cref{new-convex} for specific utility functions, their method does not apply to arbitrary CCH utility functions.

\begin{theorem}
\label{new-convex}
The optimal solution $(\allocation^*, \price^*)$ to the primal and dual of the following convex programs corresponds to equilibrium allocations and prices, respectively, of the CCH Fisher market $(\util, \budget)$:
%
\begin{equation*}
\begin{aligned}[c]
    &\text{\textbf{Primal}} \\  
    & \max_{\allocation \in \R_+^{\numbuyers \times \numgoods}} & \sum_{\buyer \in \buyers} \left[ \budget[\buyer] \log{\util[\buyer]\left(\frac{\allocation[\buyer]}{\budget[\buyer]}\right)} + \budget[\buyer] \right] \\
    & \text{subject to} & \sum_{\buyer \in \buyers} \allocation[\buyer][\good] & \leq 1 &&\forall \good \in \goods\\
    % && \allocation[\buyer][\good] &\geq 0 &&\forall \buyer \in \buyers, \good \in \goods 
\end{aligned}
\quad \vline \quad
\begin{aligned}[c]
    &\text{\textbf{Dual}} \\  &\min_{\price \in \R^\numgoods_+} \sum_{\good \in \goods} \price[\good] - \sum_{\buyer \in \buyers} \budget[\buyer] \log{ \left( \partial_{\goalutil[\buyer]}{\expend[\buyer] (\price, \goalutil[\buyer])} \right)}
\end{aligned}
\end{equation*}

% \amy{wait, is this theorem really correct? can you really just drop this term: $\sum_{\buyer \in \buyers} \budget[\buyer]\log \budget[\buyer]$. the eqm prices are the same, but i don't think it is accurate to call this the actual dual of the EG program, since its objective value does not equal the objective value of the dual.}
\end{theorem}

The proof of this theorem depends on the following lemma, whose proof can be found in \Cref{sec:Proofs4}.

\begin{lemma}
\label{differ-const}
Given a CCH Fisher market $(\util, \budget)$,
the dual of our convex program (\Cref{new-convex}) and that of Eisenberg Gale differ by a constant, namely $\sum_{\buyer \in \buyers} \left( \budget[\buyer] \log \budget[\buyer] -  \budget[\buyer] \right)$.
%
In particular,
%
\begin{align*}
\min_{\price \in \R^\numgoods_+} \left\{\sum_{\good \in \goods} \price[\good] - \sum_{\buyer \in \buyers} \budget[\buyer] \log{ \left( \partial_{\goalutil[\buyer]}{\expend[\buyer] (\price, \goalutil[\buyer])} \right)} \right\}
&=
\min_{\price \in \R^\numgoods_+} \sum_{\good \in \goods} \price[\good] + \sum_{\buyer \in \buyers} \left( \budget[\buyer] \log{ \left( \indirectutil[\buyer](\price, \budget[\buyer]) \right)} - \budget[\buyer] \right)
- \sum_{\buyer \in \buyers} \left(  \budget[\buyer] \log \budget[\buyer] - \budget[\buyer] \right)
\end{align*}
\end{lemma}

\begin{proof}[\Cref{new-convex}]
By Lemma~\ref{differ-const}, our dual and the Eisenberg-Gale dual differ by a constant, which is
%$\sum_{\buyer \in \buyers} \budget[\buyer]\log \budget[\buyer] - \sum_{\buyer \in \buyers} \budget[\buyer]$
independent of the decision variables $\price \in \R^\numgoods_+$.
Hence, the optimal prices $\price^*$ of our dual are the same as those of the Eisenberg-Gale dual, and thus correspond to equilibrium prices in the CCH Fisher market $(\util, \budget)$.
Finally, 
%since our dual differs from Eisenberg-Gale's by a constant factor, namely $\sum_{\buyer \in \buyers} \left( \budget[\buyer] \log \budget[\buyer] - \budget[\buyer] \right)$,
the objective function of our convex program's primal is:
%
\begin{align*}
    \sum_{\buyer \in \buyers}  \budget[\buyer] \log{\left(\util[\buyer] \left( \allocation[\buyer]\right) \right)} - \sum_{\buyer \in \buyers} \left( \budget[\buyer] \log \budget[\buyer] - \budget[\buyer] \right) = \sum_{\buyer \in \buyers}  \budget[\buyer] \log{\util[\buyer] \left( \frac{\allocation[\buyer]}{\budget[\buyer ]}\right)} + \sum_{\buyer \in \buyers} \budget[\buyer] \enspace .
\end{align*}
%giving the desired result.
\end{proof}

Our new convex program for CCH Fisher markets, which characterizes equilibrium expenditure functions, makes plain the duality structure between utility functions and expenditure functions that is used to compute ``shadow'' prices for allocations.
In particular, $\expend[\buyer](\price, \goalutil[\buyer])$ is the Fenchel conjugate of the indicator function $\chi_{\{\x: \util[\buyer](\allocation[\buyer]) \geq \goalutil[\buyer]\}}$, 
%i.e., $\expend[\buyer](\price, \goalutil[\buyer]) = \chi^*_{\{\x: \util[\buyer](\allocation[\buyer]) \geq \goalutil[\buyer]\}}$, where $\chi^*$ is the Fenchel conjugate of $\chi$~\cite{duality-economics}, 
meaning the utility levels and expenditures are dual (in a colloquial sense) to one another.
Therefore, equilibrium utility levels can be determined from equilibrium expenditures, and vice-versa, which implies that allocations and prices can likewise be derived from one another through this duality structure.%
\footnote{A more in-depth analysis of this duality structure can be found in \citeauthor{duality-economics} \cite{duality-economics}.
% \amy{don't use citations as nouns}
}


==> todo.tex <==
List of things to do:

\begin{enumerate}
\end{enumerate}

List of thing modified please check:

\begin{enumerate}
\end{enumerate}

